Ages and metallicities of quiescent galaxies: confronting broadband ($UVJ$) colours with stellar absorption lines

For decades, studying quiescent galaxies beyond $z\sim1$ has been challenging due to the reliance on photometric spectral energy distributions, which are highly susceptible to degeneracies between age, metallicity, dust, and star-formation history. Only recently has deep, rest-frame, optical spectroscopy made robust metallicity and age measurements possible, allowing us to empirically assess their effects on continuum shapes. To this end, we measure ages and metallicities of $\sim700$ massive ($10.2\lesssim\log(M_*/M_\odot)\lesssim11.8$), quiescent galaxies at $0.6\lesssim z\lesssim1.0$ from the Large Early Galaxy Astrophysics Census (LEGA-C) via continuum-normalized, absorption-line spectra, and compare with independent rest-frame $U-V$ and $V-J$ colours. Age increases along the quiescent sequence as both colours redden, consistent with stellar population synthesis (SPS) model predictions. Metallicity increases perpendicularly to the age trend, with higher metallicities at redder $U-V$ and bluer $V-J$ colours. Thus, age and metallicity behave differently in the $UVJ$ diagram. Moreover, this trend conflicts with SPS model expectations of increasing metallicity approximately along the quiescent sequence. Independent dynamical mass-to-light ratio trends also differ dramatically from SPS model predictions. These results demonstrate that relying on model fits to continuum shapes alone may lead to systematic biases in ages, metallicities, and stellar masses. The cause of these data-model disparities may stem from non-solar abundance patterns in quiescent galaxies or the treatment of evolved stellar phases in the models. Resolving these discrepancies is crucial, as photometric data remain central even with JWST.

==> ReadMe <==
                                                      (C.M. Cheng, 2025)
================================================================================
Ages and metallicities of quiescent galaxies: confronting broadband (UVJ) colors
with stellar absorption lines
    C.M. Cheng, et al.
    =References ?
================================================================================
Keywords: galaxies: abundances -- galaxies: fundamental parameters --
          galaxies: stellar content

Objects:
    -----------------------------------------
       RA   (2000)   DE    Designation(s)
    -----------------------------------------

Abstract:
  For decades, studying quiescent galaxies beyond $z\sim1$ has been challenging
  due to the reliance on photometric spectral energy distributions (SEDs), which
  are highly susceptible to degeneracies between age, metallicity, dust, and
  star-formation history (SFH).  Only recently has deep, rest-frame, optical
  spectroscopy made robust metallicity and age measurements possible, allowing
  us to empirically assess their effects on continuum shapes.  To this end, we
  measure ages and metallicities of ~700 massive (10.2 ~< log(M_*/M_sun) ~<
  11.8), quiescent galaxies at 0.6 ~< z ~< 1.0 from the Large Early Galaxy
  Astrophysics Census (LEGA-C) via continuum-normalized, absorption-line
  spectra, and compare with independent rest-frame U-V and V-J colours.  Age
  increases along the quiescent sequence as both colours redden, consistent with
  stellar population synthesis (SPS) model predictions.  Metallicity increases
  perpendicularly to the age trend, with higher metallicities at redder U-V and
  bluer V-J colours.  Thus, age and metallicity behave differently in the $UVJ$
  diagram.  Moreover, this trend conflicts with SPS model expectations of
  increasing metallicity approximately along the quiescent sequence.
  Independent dynamical mass-to-light ratio trends also differ dramatically from
  SPS model predictions.  These results demonstrate that relying on model fits
  to continuum shapes alone may lead to systematic biases in ages,
  metallicities, and stellar masses.  The cause of these data-model disparities
  may stem from non-solar abundance patterns in quiescent galaxies or the
  treatment of evolved stellar phases in the models.  Resolving these
  discrepancies is crucial, as photometric data remain central even with JWST.

Description:
  This catalogue contains the relevant new data for a subsample of 683 LEGA-C
  quiescent galaxies presented in this paper.  We include U-V and V-J colours
  redetermined using EAZY (Brammer et al. 2008) based on spectroscopic
  redshifts.  We also include spectroscopic ages, metallicities, and [Mg/Fe]
  abundances, derived by fitting alf (Conroy & van Dokkum 2012, Conroy et al.
  2018) to continuum-normalized absorption-line spectra.

File Summary:
--------------------------------------------------------------------------------
 FileName    Lrecl   Records    Explanations
--------------------------------------------------------------------------------
ReadMe           80        .  this file
age_met_cat.dat 267      683  


--------------------------------------------------------------------------------
Byte-by-byte Description of file: age_met_cat.dat
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
  1- 11   A11    ---    SPECT_ID  Object ID (Mask_ID).
 13- 18   I6     ---    LEGAC_ID [4949/261268] LEGA-C object ID.  Equivalent to
                               UltraVISTA.
 20- 23   A4     ---    mask      LEGA-C mask number (M#).
 25- 42   F18.14 ---    RA       [149.44/150.76] RAJ2000 (degrees) from LEGA-C.
 44- 61   F18.16 ---    DEC      [1.75/2.81] DECJ2000 (degrees) from LEGA-C.
 63- 68   F6.4   ---    z        [0.54/1.04] Spectroscopic redshift from LEGA-C.
 70- 80   F11.9  ---    UmV      [1.5/2.25] U-V colour.  U and V colours were
                               re-derived in EAZY using the spectroscopic
                               redshifts.
 82- 92   F11.9  ---    VmJ      [0.73/1.5] V-J colour.  V and J colours were
                               re-derived in EAZY using the spectroscopic
                               redshifts.
 94-111   F18.16 ---    age      [1.04/8.58] SSP-equivalent age derived from alf
                               (Gyr).
113-130   F18.16 ---    age-     [0.03/3.5] Lower uncertainty on the SSP-
                               equivalent age.
132-149   F18.16 ---    age+     [0.04/3.28] Upper uncertainty on the SSP-
                               equivalent age.
151-169   F19.16 ---    feh      [-0.96/0.3] [Fe/H] derived from alf.
171-188   F18.16 ---    feh-     [0.01/0.44] Lower uncertainty on [Fe/H].
190-207   F18.16 ---    feh+     [0.01/0.33] Upper uncertainty on [Fe/H].
209-227   F19.16 ---    mgfe     [-0.06/0.6]? [Mg/Fe] derived from alf.
229-247   F19.16 ---    mgfe-    [0.02/0.22]? Lower uncertainty on [Mg/Fe].
249-267   F19.16 ---    mgfe+    [0.02/0.26]? Upper uncertainty on [Mg/Fe].

--------------------------------------------------------------------------------



See also:
 http://... : Cheng et al. 2025.


Acknowledgements:

References:
================================================================================
     (prepared by author  / pyreadme )

